A Dual-Perspective Approach to Evaluating Feature Attribution Methods

Feature attribution methods attempt to explain neural network predictions by identifying relevant features. However, establishing a cohesive framework for assessing feature attribution remains a challenge. There are several views through which we can evaluate attributions. One principal lens is to observe the effect of perturbing attributed features on the model's behavior (i.e., faithfulness). While providing useful insights, existing faithfulness evaluations suffer from shortcomings that we reveal in this paper. In this work, we propose two new perspectives within the faithfulness paradigm that reveal intuitive properties: soundness and completeness. Soundness assesses the degree to which attributed features are truly predictive features, while completeness examines how well the resulting attribution reveals all the predictive features. The two perspectives are based on a firm mathematical foundation and provide quantitative metrics that are computable through efficient algorithms. We apply these metrics to mainstream attribution methods, offering a novel lens through which to analyze and compare feature attribution methods.

==> chapters/method_theory.tex <==
\section{About Theory}
% \usepackage{comment}
\newcommand{\kk}[1]{\noindent \fbox{\parbox{\columnwidth}{\color{red} KK: #1}}}
\subsection{Reference: Suggestion of Soundness Theorem}
Many thanks to your theorem for soundness. It is very clear and elegant compared to my old theorem, which is incorrect and wordy (contains multiple lemmas). Moreover, I am able to analyze the current implementation with the approach you used in the new theorem. I worked on your theorem and had some comments on how to adjust it to best fit our paper (and our implementation). But before I start, here is your suggestion for reference:

\kk{The original lemma 3.2 and Theorem 3.2 were incorrectly based on Assumption 1. We need the following modified assumption to conclude the original lemma 3.2 and Theorem 3.2. This is because $|\sI_v|=|\sA \cap \sI|$ does not imply $\sI_v \subseteq \sA$. The equation of $|\sI_v|=|\sA\cap \sI|$ can hold without $\sI_v \subseteq \sA$ even if $\sI_v \subseteq \sI$ and $\sA \subseteq \sI$. I fixed it by using the modified assumption.}
\kk{Instead of only fixing it, I also improved the theorem by removing the assumption of $\sA^* \cap (\sF \setminus \sI) = \emptyset$. Removing this assumption is good since it is disconnected from what is done in the actual method. I essentially prove that the minimization of $|\sA^*|$ implies this assumption without assuming it. Please notice that this is not why Assumption \ref{assumption:2}  is needed. Assumption \ref{assumption:2}  is needed to fix the proofs of the original lemma 3.2 and Theorem 3.2. So, even without this improvement of the statement of the theorem, we still need Assumption \ref{assumption:2}.}
\begin{assumption}\label{assumption:2}
    $\forall  \sF_1, \sF_2 \subseteq \sF$, if $\rho(f(\sF_1)) < \rho(f(\sF_2))$, then $|\sI_v \cap \sF_1| < |\sI_v \cap \sF_2|$.
\end{assumption}
\begin{theorem} \label{theorem:soundness}
    Suppose that $\sS_v(\sA)=\{\sS \subseteq \sA: \rho(f(\sI_v)) = \rho(f(\sS))\}$ is not empty. Let $\sA^* \in \arg\min_{\sS \in \sS_v(\sA)} |\sS| \subseteq \sA$. Then, the soundness of $\sA$ at information level $v$  is $\frac{|\sA^*|}{|\sA|}$.
\end{theorem}
\textbf{Proof}: For any $\sS \in \sS_v(\sA)$ including $\sA^*$, using Assumption \ref{assumption:2} and the condition of $\rho(f(\sI_v)) = \rho(f(\sS))$, we have that $|\sI_v|=|\sI_v \cap \sI_v| = |\sS \cap \sI_v|= |\sS| - |\sS \cap (\sF \setminus \sI_v)|$. Since $\varphi(F) > 0$ for all $F \in \mathcal{I}$, this implies that $\sI_v \subseteq \sS$ and $|\sS|=|\sI_v|+ |\sS \cap (\sF \setminus \sI_v)|$. Thus, $\min_{\sS \in \sS_v(\sA)} |\sS|= \min_{\sS \in \sS_v(\sA)} |\sS \cap (\sF \setminus \sI_v)|=0$ where the first equality is due to $|\sS|=|\sI_v|+ |\sS \cap (\sF \setminus \sI_v)|$ and the second equality follows from $\sI_v \subseteq \sS$ (since $\sI_v \subseteq \sS$ implies that $\sI_v \in \sS_v(\sA)$).
Thus, from the definition of $\sA^*$, we have $|\sA^* \cap (\sF \setminus \sI_v)|=0$ and therefore $|\sA^*|=|\sI_v|+|\sA^* \cap (\sF \setminus \sI_v)|=|\sI_v|$. Since $|\sI_v|=|\sS \cap \sI_v|$ for all $\sS \in \sS_v(\sA)$ including $\sA^*$ (see above), this implies that $|\sA^*|=|\sI_v|=|\sA^* \cap \sI_v|$. \qed

\subsection{Limitation of the Previous Theorems of Soundness and Completeness}
Right now to derive the theorem for soundness, we need one additional assumption \ref{assumption:2}. However, we have made a similar assumption before:
\begin{assumption}\label{neural_network_assumption}\label{assumption}
    Given a dataset $\mathbb D$, let $\sF$ be the set of all input features in $\mathbb D$, $f$ be a model, and $\rho$ be a performance metric to assess the performance of model $f$. $\forall  \sF_1, \sF_2 \subseteq \sF$, if $\rho(f(\sF_1)) < \rho(f(\sF_2))$, then $|\sI \cap \sF_1|_I < |\sI \cap \sF_2|_I$, where $\sI \subseteq \sF$ is the set of informative features for model $f$.
\end{assumption}

The only difference between these two assumptions is the use of $\sI$ and $\sI_v$. Actually, using $\sI_v$ would make the assumption too strong. This means for every possible $\sI_v$, the model performance $\rho(f(\cdot))$ can always be used to compare $|\sI_v \cap \sF_1|$ and $|\sI_v \cap \sF_2|$. Hence, comparing $|\sI \cap \sF|$ makes more sense, as $\sI$ represents the set of all informative features.

I then realized that here we are using a strong assumption to make a conclusion that is also too strong. Here, we are saying that we can calculate soundness for every possible $\sI_v$, so readers can easily argue which $\sI_v$ makes more sense. Below, I present a modified theorem that is more related to our implementation. The idea is to eliminate both $\sI_v$ and Assumption \ref{assumption:2}, then use Assumption \ref{neural_network_assumption} during derivation. I also fixed many issues of my previous ambiguous definition.

\subsection{Modified Theorem for Soundness and Completeness}
We first define two norm operators. For any set $\sS$ of features, $|\sS|_I=\sum_{F \in \sS} \varphi(F)$ where $\varphi(F) \ge 0$ is the information of the feature $F$ such that $\varphi(F) > 0$ for all $F \in \sI$. Analogously, $|\sS|_A=\sum_{F \in \sS} \eta(F)$ where $\eta(F) \ge 0$ is the attribution value of the feature $F$ such that $\eta(F) > 0$ for all $F \in \sA$.
\begin{definition}
    The soundness of an attribution set $\sA$ is the ratio of informative attribution to total attribution, i.e., $\frac{|\sA\cap\sI|_A}{|\sA|_A}$.
\end{definition}
\begin{definition}
    The completeness of an attribution set $\sA$ is the ratio of attributed information to total information, i.e., $\frac{|\sA\cap\sI|_I}{|\sI|_I}$.
\end{definition}
You may notice that they use two norms separately. We can provide a simple argument to show why this is essential. Assume we calculate soundness as $\frac{|\sA\cap\sI|_I}{|\sA|_I}$, this is actually 1. Moreover, $\frac{|\sA\cap\sI|_A}{|\sI|_A}$ is also always 1.
\subsubsection{Soundness}
\begin{theorem} \label{theorem:soundness}
    Suppose that $\sS_v(\sAinc)=\{\sS \subseteq \sAinc: \rho(f(\sAinc)) = \rho(f(\sS))\}$ is not empty for any $\sAinc \subseteq \sA$. Let $\sA^* \in \arg\min_{\sS \in \sS_v(\sAinc)} |\sS|_A \subseteq \sAinc$. Then, the soundness of $\sAinc$ is $\frac{|\sA^*|_A}{|\sAinc|_A}$.
\end{theorem}
\textbf{Proof}: For any $\sS \in \sS_v(\sAinc)$ including $\sA^*$, Assumption \ref{neural_network_assumption} and the condition $\rho(f(\sAinc)) = \rho(f(\sS))$ imply that $|\sAinc \cap \sI|_I = |\sS \cap \sI|_I$. Note that $\sS \subseteq \sAinc$ implies $|\sS\cap\sI|_I\leq |\sAinc\cap\sI|_I$, with the equality being achieved when $\sS\cap\sI = \sAinc\cap\sI$.  Therefore, $\sS\cap\sI = \sAinc\cap\sI$. Besides, the minimization problem $\min_{\sS \in \sS_v(\sAinc)} |\sS|_A= \min_{\sS \in \sS_v(\sA)} (|\sS \cap \sI|_A + |\sS \cap (\sF \setminus \sI)|_A)$ boils down to $\min_{\sS \in \sS_v(\sA)}|\sS \cap (\sF \setminus \sI)|_A$, because $\sS\cap\sI = \sAinc\cap\sI$ implies $|\sS\cap\sI|_A = |\sAinc\cap\sI|_A$, which is a constant with fixed $\sAinc$.
Thus, according to the definition of $\sA^*$, we have $|\sA^* \cap (\sF \setminus \sI)|_A = 0$ and therefore $|\sA^*|_A=|\sAinc \cap \sI|_A+|\sA^* \cap (\sF \setminus \sI)|_A=|\sAinc\cap\sI|_A$. $|\sA^* \cap (\sF \setminus \sI)|_A=0$ indicates $\sA^*\subseteq\sI$ since $ \eta(F) > 0$ holds for all $F \in \sA^* \subseteq \sA$. Next, $\sA^*\subseteq\sI$ and $\sA^*\subseteq\sAinc$ yields $\sA^* \subseteq (\sAinc \cap \sI)$. Combining with $|\sA^*|_A = |\sAinc \cap\sI|_A$, we have $\sA^* = \sAinc\cap\sI$. Therefore, the soundness of $\sAinc$ is $\frac{|\sAinc\cap\sI|_A}{|\sAinc|_A} = \frac{|\sA^*|_A}{|\sAinc|_A}$. \qed



\subsubsection{Completeness}
The completeness theorem is identical as before, we just update it with the actual norm $|\cdot|_I$.
\begin{theorem} \label{theorem:completeness}
    Assume two attribution methods with returned salient features $\sA_1$ and $\sA_2$, respectively. If $\rho(f(\sF \setminus \sA_1)) < \rho(f(\sF \setminus \sA_2))$, then the attribution method associated with $\sA_1$ is more complete than the one associated with $\sA_2$.
\end{theorem}
\textbf{Proof}: The condition of $\rho(f(\sF \setminus \sA_1)) < \rho(f(\sF\setminus \sA_2))$ together with Assumption \ref{assumption} implies that $|\sI \cap (\sF \setminus \sA_1)|_I<|\sI \cap (\sF \setminus \sA_2)|_I$. Here, for any set $\sS$, $|\sI \cap (\sF \setminus \sS)|_I=\sum_{F \in (\sI \cap (\sF \setminus \sS))} \varphi(F) = \sum_{F \in \sI} \varphi(F) - \sum_{F \in (\sI \cap \sS)} \varphi(F)=|\sI|_I-|\sI \cap \sS|_I$. Using this for $\sS = \sA_1$ and $\sA_2$, we have that $|\sI \cap (\sF \setminus \sA_1)|<|\sI \cap (\sF \setminus \sA_2)| \Leftrightarrow |\sI|-|\sI \cap \sA_1| < |\sI|-|\sI \cap \sA_2| \Leftrightarrow \frac{|\sI \cap \sA_2|}{|\sI|} < \frac{|\sI \cap \sA_1|}{|\sI|}$. \qed
